Learning New Tasks from a Few Examples with Soft-Label Prototypes

Existing approaches to few-shot learning in NLP rely on large language models (LLMs) and/or fine-tuning of these to generalise on out-of-distribution data. In this work, we propose a novel few-shot learning approach based on soft-label prototypes (SLPs) designed to collectively capture the distribution of different classes across the input domain space. We focus on learning previously unseen NLP tasks from very few examples (4, 8, 16) per class and experimentally demonstrate that our approach achieves superior performance on the majority of tested tasks in this data-lean setting while being highly parameter efficient. We also show that our few-shot adaptation method can be integrated into more generalised learning settings, primarily meta-learning, to yield superior performance against strong baselines.

==> sections/related_work-OLD.tex <==
\section{Related work}

% few-shot learning and history of bert
Few-shot learning in NLP \cite{bert,text-to-text-transformer,albert,zhuang-etal-2021-robustly} has recently consisted of fine-tuning pretrained encoder language models on specific tasks in a supervised learning paradigm to leverage excellent performance. As most few-shot supervised learning methods in NLP consist of a base pre-trained encoder (BERT \cite{bert}, ROBERTA \cite{roberta}, ALBERT \cite{albert}), we consider BERT\textsubscript{base} \cite{bert} as the pre-trained encoder for all our methods. 

\paragraph{Meta-learning} For encoder-based models, meta-learning has emerged as a viable methodology for few-shot learning. 
In the meta-learning paradigm, the training and test sets, referred to as $\mathcal{D}$\textsubscript{meta-train} and $\mathcal{D}$\textsubscript{meta-test}, are split into episodes. Each episode encompasses a task $\mathcal{T}$\textsubscript{i} and consists of a support set $\mathcal{D}^{(i)}$\textsubscript{support} and a query set $\mathcal{D}^{(i)}$\textsubscript{query}. Meta-learning algorithms initially fit the model on the support set of the episode (inner-loop optimisation) and then achieve generalisation across episodes by optimising performance on the query sets of the episodes (outer-loop optimisation). For evaluation, the model is first fine-tuned on the support set and then evaluated on the query set for each task $\mathcal{T}$\textsubscript{i} $\in$ $\mathcal{D}$\textsubscript{meta-test}. We describe the process algorithmically in Algorithm \ref{alg:meta-learning} and describe the \textit{MetaUpdate} process for different algorithms subsequently.

\begin{algorithm}[h]
\caption{Meta-learning}\label{alg:meta-learning}
$\alpha, \beta \leftarrow$ learning rates \\
Sample batch of tasks $\{T_i\} \sim p(T)$ \\ 
Initialise $\mathbf{\theta'_i} \leftarrow \theta$ \\
\For{$T_i \sim p(T)$}{
    Partition $T_i$ into $D^s_i$ and $D^q_i$ \\  
    $\mathbf{\theta'_i} \leftarrow \mathbf{\theta} - \alpha\nabla_\theta\mathcal{L}^s_{\mathcal{D}_i}(f_\theta)$ for $k$ steps\\ 
}
$\theta \leftarrow$ MetaUpdate$(\theta_i, D_i^q, \beta)$ \\
\end{algorithm}

\paragraph{Model Agnostic Meta-Learning} MAML \cite{maml} is an \textit{optimisation-based} meta-learning approach which incorporates generalisability across tasks in its cost function. The task loss $\mathcal{L}^q_{\mathcal{T}_i}$ is computed on the query examples in each episode, using this task-specific model. The initial model parameters $\theta$ are then updated so as to minimize the sum of the losses of all tasks in a batch, leading to improved generalisation across tasks. The \textit{MetaUpdate} step is thus defined as 

$$
\mathbf{\theta} \leftarrow \mathbf{\theta} - \beta\:\nabla_\theta\sum_{\mathcal{T}_i \sim p(\mathcal{T})}\mathcal{L}^q_{\mathcal{D}_i}(f_{\theta_i'})
$$

Note that the \textit{MetaUpdate} expression calculates the gradients of each $\theta_i$ with respect to $\theta$, thus necessitating the computation of second-order gradients. To ease computation, we use a first-order approximation of MAML (FOMAML) wherein the gradients of each $\theta_i$ are calculated with respect to $\theta_i$ and reduce the \textit{MetaUpdate} term to 

$$
\mathbf{\theta} \leftarrow \mathbf{\theta} - \beta\:\nabla_{\theta_i}\sum_{\mathcal{T}_i \sim p(\mathcal{T})}\mathcal{L}^q_{\mathcal{D}_i}(f_{\theta_i'})
$$

\paragraph{LEOPARD} 

\citet{leopard} employ meta-learning for diverse NLP tasks in an approach inspired from MAML which integrates a text encoder model with a meta-learned parameter generator to tailor task-specific initialisations for the classification head. Their inner-loop update learns the parameter generator for the task, adapts task-specific model parameters and the \textit{MetaUpdate} step adapts model parameters as done in MAML. They show that their method, LEOPARD, outperforms multi-task trained models as well as a range of other meta-learning methods. 

\paragraph{Reptile} This meta-learning algorithm, introduced by \citet{reptile}, is computationally simple compared to MAML and LEOPARD - the \textit{MetaUpdate} step simply moves the model parameters towards inner-loop finetuned model parameters, thus assuming the form

$$
\theta \leftarrow \theta + \beta \frac{1}{|\{T_i\}|}\sum_{T_i \sim p(T)}(\theta_i - \theta)
$$

Despite it's simplicity, it reports strong performances on a variety of few-shot learning tasks \cite{meta-learning-dou}.

\paragraph{Prototypical Networks} Unlike optimisation-driven meta-learning methods, Prototypical Networks \cite{proto-net} is a metric-based meta-learning method that uses an embedding function $f_{\theta}$ to encode training support samples and compute a high-dimensional vector $\mu _c$ that is the arithmetic mean of the training data points of class $c$. It then uses a distance function $d$ to compute the similarity between a query instance $x$ and the mean vector of each class to get the class distribution as: 
\begin{gather*}
    p(y=c|x) = softmax(-d(f_\theta (x), \mu _c)) \\ 
    = \frac{exp(-d(f_\theta(x),\mu_c))}{\sum_{c' \in C}exp(-d(f_\theta(x),\mu_c'))}
\end{gather*}
Model optimisation is done using the loss function $J(\mathbf{\theta}) = -log(p(y = c^*|x,\theta))$.

\paragraph{Generative language models} Another line of research in LLMs has been pre-training decoder-only large language models (GPT4 \cite{gpt4}, Llama \cite{llama}, Bloom \cite{bloom} etc.) on language modelling tasks using a massive amount of textual data available on the internet. These text-generative models, compared to language encoder models, are much larger in size with parameters often running into hundreds of billions. Few-shot learning in these models conforms to the \textit{in-context learning} paradigm \cite{min-etal-2022-rethinking, gpt3, prompting-gpt3} wherein a language task is initially reduced to a language generation task and the predictions of this generated task are evaluated after being exposed to a few examples. In-context learning reports strong performance in a variety of linguistic tasks such as text classification, natural language inference and semantic parsing \cite{gpt3, liu-etal-2022-makes, pmlr-v139-zhao21c}. Though generative LLMs are strong performers, they are unsuitable for our test tasks for the following reasons - 
\begin{itemize}
    \item Our method relies on training text encoders which can generate compact representations at the phrase level - a pre-training task that generative LLMs are not trained on. 
    \item To the best of our knowledge, all state-of-the-art open-source generative LLMs are trained on textual data available on Github, where our test tasks are available as well\footnote{\url{https://github.com/iesl/leopard}}. Our investigations reveal that there is significant data leakage and all state-of-the-art generative LLMs have already been exposed to our test data - thus using them as a base model would lead to an incorrect evaluation.
    \item Generative LLMs require massive computational resources which are prohibitively expensive in our case. To demonstrate the power of our method, we use (comparatively) computationally cheaper encoder LLMs and demonstrate strong performances across a variety of baselines keeping our encoder uniform -- thus enabling a meaningful comparison. 
\end{itemize}


